A Cohesive Deep Drilling Field Strategy for LSST Cosmology

The Vera C. Rubin Observatory Legacy Survey of Space and Time (LSST) will image billions of astronomical objects in the wide-fast-deep primary survey and in a set of minisurveys including intensive observations of a group of deep drilling fields (DDFs). The DDFs are a critical piece of three key aspects of the LSST Dark Energy Science Collaboration (DESC) cosmological measurements: they provide a required calibration for photometric redshifts and weak gravitational lensing measurements and they directly contribute to cosmological constraints from the most distant type Ia supernovae. We present a set of cohesive DDF strategies fulfilling science requirements relevant to DESC and following the guidelines of the Survey Cadence Optimization Committee. We propose a method to estimate the observing strategy parameters and we perform simulations of the corresponding surveys. We define a set of metrics for each of the science case to assess the performance of the proposed observing strategies. We show that the most promising results are achieved with deep rolling surveys characterized by two sets of fields: ultradeep fields (z<1.1) observed at a high cadence with a large number of visits over a limited number of seasons; deep fields (z<0.7), observed with a cadence of ~3 nights for ten years. These encouraging results should be confirmed with realistic simulations using the LSST scheduler. A DDF budget of ~8.5% is required to design observing strategies satisfying all the cosmological requirements. A lower DDF budget lead to surveys that either do not fulfill photo-z/WL requirements or are not optimal for SNe Ia cosmology.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main ?= main
#default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname ?= $(notdir $(shell pwd))

#ifeq ($(default), {{ cookiecutter.default_format }})
style ?= lsstdescnote
#else
# style=${default}
#endif

# 'note' shall be an alias for 'lsstdescnote'
ifeq ($(style),note)
style = lsstdescnote
endif
# mkauthlist doesn't recognize lsstdescnote as a style, so tell it to do something generic
ifeq ($(style),lsstdescnote)
mastyle = tex
else
mastyle = $(style)
endif

DESCTEX := desc-tex
DESCTEXORIGIN := https://github.com/LSSTDESC/desc-tex.git
LSSTTEX := lsst-texmf
LSSTTEXORIGIN := https://github.com/lsst/lsst-texmf.git

localpip ?= F
PIPOPTS = --upgrade-strategy only-if-needed
ifeq ($(localpip),T)
MKAUTHBIN := bin/mkauthlist
MKAUTH := PYTHONPATH=$$(ls -d lib/python*/site-packages 2>/dev/null | head -n1):$$PYTHONPATH $(MKAUTHBIN)
PIPOPTS += --install-option="--prefix=$(PWD)"
GETMKAUTH := [ -e $(MKAUTHBIN) ] || pip install $(PIPOPTS) mkauthlist
else
MKAUTHBIN :=
MKAUTH := mkauthlist 
GETMKAUTH := pip list 2>/dev/null | grep -q mkauthlist || pip install $(PIPOPTS) mkauthlist
endif

# LATEX environment variables
export TEXINPUTS:=./$(DESCTEX)/styles/:./tables/:
export BSTINPUTS:=./$(DESCTEX)/bst/:
export BIBINPUTS:=./$(DESCTEX)/bib/:./$(LSSTTEX)/texmf/bibtex/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir := tmp
figdir ?= ./figures
figures ?= $(figdir)/*.{png,jpg,pdf}
tabdir ?= ./tables
tables ?= $(tabdir)/*.tex
styles ?= ./$(DESCTEX)/styles/*.{sty,cls}
bibs ?= ./$(DESCTEX)/bib/*.bst
source = $(main).{tex,bbl,bib} $(DESCTEX)/bib/lsstdesc.bib $(DESCTEX)/ack/*.tex authors.tex contributions.tex $(LSSTTEX)/texmf/bibtex/bib/lsst.bib $(LSSTTEX)/texmf/bibtex/bib/lsst-dm.bib

tarfiles = $(figures) $(tables) $(styles) $(bibs) $(source)

# prefix for difference files
DIFPRE ?= diff_
# git repo branch to compare changes against
BASEBRANCH ?= master
# git repo branch we are compiling
THISBRANCH := $(shell git branch --no-color 2> /dev/null | sed -e '/^[^*]/d' -e 's/* \(.*\)/ \1/' | tr -d ' ')
# temp file for the version to compare against
DRAFT = $(main).$(BASEBRANCH)
# base for difference files to generate
DIFF = $(DIFPRE)$(THISBRANCH)--$(BASEBRANCH)


maketargets := all authlist clean copy diff help $(main) update tar templates tidy touch
.PHONY: $(maketargets)

styleopts := aastex61 apj apjl emulateapj lsstdescnote mnras note prd prl tex 
help:
	@echo "Usage: make [style=lsstdescnote] [localpip=F] <target(s)>\n Possible targets: $(maketargets) <style> $(DESCTEX) $(LSSTTEX)\n  all: equivalent to 'make $(main) copy'\n  authlist: use mkauthlist to generate latex author/affiliation listing\n  clean: remove latex temporary files AND compiled outputs\n  copy: copy $(main).pdf to $(outname).pdf\n  diff: if we're in a git repo, use latexdiff to compare the current $(main).tex vs the $(BASEBRANCH) branch, and attempt to compile to $(DIFF).pdf\n  help: what you're looking at\n  $(main): compile $(main).tex\n  update: update desc-tex, mkauthlist, and templates repo\n  tar: tar up latex source files to $(outname).tar.gz\n  templates: download latest templates to templates/\n  tidy: delete latex temporary files\n  touch: touch $(main).tex to force a recompile\n  <style>: equivalent to 'make style=<style> $(main) copy tar' (see style option)\n  $(DESCTEX): download $(DESCTEX), which provides the DESC header logo and latex helper files (done automatically on first latex compilation)\n  $(LSSTTEX): download $(LSSTTEX), providing (among other things) LSST project bib files (not done automatically)\n Options for style: $(styleopts) (Anything else results in generic latex)\n Options for localpip: T or F. Set to T to install mkauthlist in this directory rather than systemwide"


# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
$(main): export flag = \def\flag{${style}}
envflag = \\def\\flag{${style}}
all: $(main) copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

# if we are in a git repo, add as a submodule; otherwise clone
$(DESCTEX):
	if [ -d .git ]; then git submodule add $(DESCTEXORIGIN); else git clone $(DESCTEXORIGIN); fi
$(LSSTTEX):
	if [ -d .git ]; then git submodule add $(LSSTTEXORIGIN); else git clone $(LSSTTEXORIGIN); fi

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
$(main) : $(DESCTEX) authlist
	STYLEFLAG=$(envflag) latexmk $(main)
#	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

diff: $(DIFF).pdf
$(DIFF).pdf: $(DIFF).tex
	STYLEFLAG=$(envflag) latexmk $<
$(DIFF).tex: $(DRAFT).tex $(main).tex
	latexdiff --exclude-textcmd="multicolumn" $^ > $@
# this ensures that the version to latexdiff against is always updated
.PHONY: $(DRAFT).tex
$(DRAFT).tex:
	if git show $(BASEBRANCH):$(main).tex > $@; then true; else echo "\n\n'make diff' is intended to be used inside a git repository\n"; false; fi



tar : $(main)
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist: authors.tex
authors.tex : authors.csv
	$(GETMKAUTH)
	$(MKAUTH) -j ${mastyle} -f -c "LSST Dark Energy Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex
#	pip install --upgrade mkauthlist


# http://stackoverflow.com/q/8028314/
.PHONY: $(styleopts)
$(styleopts): export style = $(@)
$(styleopts): export flag = \def\flag{$(@)}
$(styleopts):
	$(MAKE) -e $(main)
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/deploy

# UPDATES=\
# texmf/bib/apj.bst \
# texmf/bib/mnras.bst \
# texmf/styles/aas_macros.sty \
# texmf/styles/aastex.cls \
# texmf/styles/aastex61.cls \
# texmf/styles/aps_macros.sty \
# texmf/styles/docswitch.sty \
# texmf/styles/emulateapj.cls \
# texmf/styles/mnras.cls \
# texmf/styles/lsstdescnote.cls \
# texmf/styles/lsstdesc_macros.sty \
# texmf/logos/desc-logo-small.png \
# texmf/logos/desc-logo.png \
# texmf/logos/header.png \
# lsstdesc.bib \
# .travis.yml \
# figures/example.png

# .PHONY: $(UPDATES)
# $(UPDATES):
# 	curl -s -S -o $(@) ${baseurl}/$(@)
# 	@echo " "

update: templates
	@echo Updating desc-tex
	cd $(DESCTEX) && git pull
	@echo
	@echo Updating mkauthlist
	pip install --upgrade $(PIPOPTS) mkauthlist
#@echo "\nOver-writing LaTeX style files with the latest versions: \n"
#@mkdir -p .logos figures texmf/styles texmf/bib
#$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:
# It is a bad idea to make these phony targets

TEMPLATES:=\
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
Makefile
#.metadata.json \
#.travis.yml 
#figures/example.png
# #acknowledgments.tex \

ALLTEMPLATES := $(TEMPLATES) header.png

# .PHONY: $(TEMPLATES)
# $(TEMPLATES):
# 	curl -s -S -o templates/$(@) ${baseurl}/$(@)
# 	@echo " "

gettemplates := $(foreach t,$(TEMPLATES),curl -s -S -o templates/$(t) ${baseurl}/$(t); )

# NB: fetching header.png will fail as long as desc-tex is private
templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(gettemplates)
	curl -f -s -S -o templates/header.png https://raw.githubusercontent.com/LSSTDESC/desc-tex/master/logos/header.png || true
	@echo
	@echo templates/ listing:
	@ls -a templates/*
	@for f in $(ALLTEMPLATES); do diff -q $$f templates/$$f; true; done
#$(MAKE) $(TEMPLATES)
#	$(MAKE) new

# Get a template copy of the latest Makefile, for reference:
# new:
# 	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
# 	@mkdir -p templates
# 	curl -s -S -o templates/Makefile ${baseurl}/Makefile
# 	@echo " "

# Over-write this Makefile with the latest version:
# Why would we include this when a safe option already exists?
# upgrade:
# 	@echo "\nDownloading the latest version of the Makefile: \n"
# 	curl -s -S -o Makefile ${baseurl}/Makefile
# 	@echo "\nUpgrading version of mkauthlist: \n"
# 	pip install mkauthlist --upgrade --no-deps
# 	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==
\author{Ph.~Gris}
%\affiliation{Laboratoire de Physique de Clermont (LPC) , CNRS/IN2P3, F-63000 Clermont-Ferrand, France}
\author{H.~Awan}
%\affiliation{}
\author{M.~Becker}
\author{H.~Lin}
\collaboration{(LSST Dark Energy Science Collaboration)}

==> contributions.tex <==
Author contributions are as follows. Philippe Gris: conceptualization, software, analysis, paper writing. Humna Awan: critical analysis of the work, contribution to the general optimization of the survey through builder work. Matt Becker: definition of WL requirements, paper writing. Huan Lin: definition of \photz~requirements, paper writing.


==> desc-tex/ack/key.tex <==
The DESC acknowledges ongoing support from the Institut National de 
Physique Nucl\'eaire et de Physique des Particules in France; the 
Science \& Technology Facilities Council in the United Kingdom; and the 
Department of Energy, the National Science Foundation, and the LSST 
Corporation in the United States.  DESC uses resources of the IN2P3 
Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the 
Centre National de la Recherche Scientifique; the National Energy 
Research Scientific Computing Center, a DOE Office of Science User 
Facility supported by the Office of Science of the U.S.\ Department of
Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, 
funded by UK BEIS National E-infrastructure capital grants; and the UK 
particle physics grid, supported by the GridPP Collaboration.  This 
work was performed in part under DOE Contract DE-AC02-76SF00515.


==> desc-tex/ack/standard.tex <==
The DESC acknowledges ongoing support from the Institut National de 
Physique Nucl\'eaire et de Physique des Particules in France; the 
Science \& Technology Facilities Council in the United Kingdom; and the
Department of Energy, the National Science Foundation, and the LSST 
Corporation in the United States.  DESC uses resources of the IN2P3 
Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the 
Centre National de la Recherche Scientifique; the National Energy 
Research Scientific Computing Center, a DOE Office of Science User 
Facility supported by the Office of Science of the U.S.\ Department of
Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, 
funded by UK BEIS National E-infrastructure capital grants; and the UK 
particle physics grid, supported by the GridPP Collaboration.  This 
work was performed in part under DOE Contract DE-AC02-76SF00515.


==> desc-tex/ack/standard_short.tex <==
DESC acknowledges ongoing support from the IN2P3 (France), the STFC 
(United Kingdom), and the DOE, NSF, and LSST Corporation (United States).  
DESC uses resources of the IN2P3 Computing Center 
(CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la
Recherche Scientifique; the National Energy Research Scientific Computing
Center, a DOE Office of Science User Facility supported under Contract 
No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BEIS National 
E-infrastructure capital grants; and the UK particle physics grid, supported
by the GridPP Collaboration.  This work was performed in part under DOE 
Contract DE-AC02-76SF00515.


==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex/:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'


==> res_m5.tex <==
\begin{table}[!htbp]
\begin{center}
\caption{\fivesig~values used in the simulations. These values are extracted from the LSST simulation baseline\_v3.0\_10yrs.}\label{tab:fivesigmasim}
\begin{tabular}{c|c|c}
\hline
\hline
season & band & \fivesig~single exposure\\
\hline
 &u &23.56/23.16/23.55/23.14/22.98/23.14 \\
 &g &24.21/23.68/24.21/23.12/24.30/24.32 \\
1  &r &23.91/23.33/23.73/23.04/23.82/23.61 \\
 &i &23.52/22.95/23.45/22.93/23.45/23.41 \\
 &z &22.63/22.27/22.83/22.48/22.64/22.73 \\
 &y &22.04/21.35/22.08/21.81/21.75/21.81 \\
\hline
 &u &23.39/23.14/23.57/22.90/23.76/23.77 \\
 &g &24.18/23.89/24.26/23.86/24.55/24.56 \\
2  &r &23.72/23.62/23.89/23.84/24.13/24.16 \\
 &i &23.40/23.19/23.56/23.31/23.69/23.66 \\
 &z &22.68/22.35/22.91/22.69/22.86/22.83 \\
 &y &21.83/21.83/22.05/21.82/22.16/22.25 \\
\hline
 &u &23.20/23.72/23.61/23.67/23.95/23.87 \\
 &g &23.65/24.30/24.38/24.45/24.57/24.59 \\
3  &r &23.27/23.97/24.03/24.06/24.18/24.09 \\
 &i &23.07/23.55/23.68/23.66/23.85/23.80 \\
 &z &22.57/22.95/22.90/22.89/23.21/23.08 \\
 &y &21.71/22.06/22.20/22.29/22.22/22.31 \\
\hline
 &u &23.45/22.63/23.09/23.19/23.32/23.19 \\
 &g &24.12/24.20/23.81/23.87/24.25/24.25 \\
4  &r &23.83/23.68/23.57/23.44/24.11/24.08 \\
 &i &23.39/23.41/23.22/23.45/23.55/23.51 \\
 &z &22.58/22.46/22.80/22.57/22.71/22.73 \\
 &y &21.86/21.66/22.00/21.91/21.80/21.81 \\
\hline
 &u &23.60/22.87/23.28/23.50/23.33/23.24 \\
 &g &24.17/23.27/24.39/24.40/24.42/24.39 \\
5  &r &23.79/23.35/23.88/23.68/23.89/23.83 \\
 &i &23.28/23.02/23.51/23.49/23.46/23.45 \\
 &z &22.70/22.28/22.57/22.24/22.56/22.60 \\
 &y &22.01/21.20/21.75/21.80/21.55/21.65 \\
\hline
 &u &23.31/23.08/23.41/23.51/23.45/23.55 \\
 &g &23.91/23.46/24.01/23.61/23.86/23.89 \\
6  &r &23.68/23.35/23.64/23.49/23.70/23.84 \\
 &i &23.22/23.09/23.34/23.03/23.45/23.37 \\
 &z &22.53/22.50/22.48/22.60/22.79/22.89 \\
 &y &21.67/21.37/21.79/21.98/21.99/21.97 \\
\hline
 &u &23.01/23.24/23.58/23.68/23.54/23.67 \\
 &g &23.73/24.13/24.45/24.14/24.44/24.44 \\
7  &r &23.52/23.69/23.86/23.71/23.95/24.00 \\
 &i &23.14/23.23/23.55/23.39/23.56/23.54 \\
 &z &22.49/22.76/22.49/22.74/22.52/22.59 \\
 &y &21.65/21.81/21.92/21.94/21.90/21.98 \\
\hline
 &u &22.95/23.18/22.96/23.09/23.25/23.28 \\
 &g &23.63/23.67/24.12/23.84/24.21/24.31 \\
8  &r &23.42/23.50/23.56/23.71/23.84/23.39 \\
 &i &23.05/23.17/23.55/23.28/23.53/23.41 \\
 &z &22.63/22.33/22.50/22.92/22.35/22.40 \\
 &y &21.51/21.57/22.10/22.02/21.37/21.53 \\
\hline
 &u &23.00/23.00/22.62/22.58/23.06/23.11 \\
 &g &23.21/22.94/23.86/23.35/23.31/23.28 \\
9  &r &23.23/22.87/23.75/22.97/23.24/23.22 \\
 &i &22.97/22.62/23.29/22.85/22.88/22.87 \\
 &z &22.33/21.87/22.05/22.11/22.35/22.32 \\
 &y &21.34/21.09/21.35/21.17/21.76/21.56 \\
\hline
 &u &23.60/23.41/23.27/23.10/23.08/23.14 \\
 &g &24.28/23.74/24.19/24.20/23.54/23.65 \\
10  &r &23.84/23.49/23.42/23.77/23.17/23.26 \\
 &i &23.48/23.02/23.28/23.43/23.05/23.01 \\
 &z &22.75/22.19/22.30/22.71/22.56/22.56 \\
 &y &21.98/21.53/21.60/21.70/21.81/21.92 \\
\hline
\hline
\end{tabular}
\end{center}
\end{table}

% This table was automatically generated using the command
% python run_scripts/OS_info/m5_med_season.py >> res_m5.tex
